Optimal sensor deception in stochastic environments with partial observability to mislead a robot to a decoy goal

Deception is a common strategy adapted by autonomous systems in adversarial settings. Existing deception methods primarily focus on increasing opacity or misdirecting agents away from their goal or itinerary. In this work, we propose a deception problem aiming to mislead the robot towards a decoy goal through altering sensor events under a constrained budget of alteration. The environment along with the robot's interaction with it is modeled as a Partially Observable Markov Decision Process (POMDP), and the robot's action selection is governed by a Finite State Controller (FSC). Given a constrained budget for sensor event modifications, the objective is to compute a sensor alteration that maximizes the probability of the robot reaching a decoy goal. We establish the computational hardness of the problem by a reduction from the $0/1$ Knapsack problem and propose a Mixed Integer Linear Programming (MILP) formulation to compute optimal deception strategies. We show the efficacy of our MILP formulation via a sequence of experiments.

==> introduction.tex <==
Deception is a common form of adversarial attack, which can manifest as concealing one's intent from adversary agents or misleading the adversary by manipulating their sensor information. In this paper, we focus on the latter, where a team of agents seeks to mislead an opposing team by directing them toward decoy goals through sensor manipulation. However, modifying sensor information incurs a cost, which the agents aim to minimize. This form of deception has broad applications in autonomous system planning, from game-based scenarios to military operations.
For example, consider a strategic defense scenario where an unauthorized ground robot attempts to infiltrate a protected area while avoiding detection. The adversarial home system can manipulate the sensor observations that the robot rely on, misdirecting them away from the protected area and towards a controlled or isolated region. The cost of manipulating sensor observations can include energy expenditure or the risk posed to authorized friendly agents. Another example in a game-based scenario is where one team deceives the opposing team by leading them into dead-ends or endless loops, thereby wasting valuable resources such as time. This can be achieved by manipulating navigation cues, such as swapping landmarks or signposts, to misdirect the opposing team away from the objective or prize. The cost of swapping landmarks or signposts can be the time required to carry out the alteration.

In this paper, we consider a stochastic environment and model its changes based on the behavior of the agent (or robot) being misled using a Partially Observable Markov Decision Process (POMDP). The robot does not have direct knowledge of the current state but receives observations that depend on the actual state. These observations can be altered at a cost by an adversarial agent. The robot (or the agent being misled) selects actions based on its current observations and memory, which is modeled as a Finite State Controller. The objective of the system is to minimize the sensor alteration cost for the adversarial agent while ensuring that the robot reaches one of the decoy goals with a positive probability. 

We construct the product automaton of the POMDP and FSC, to efficiently compute the probability of misleading the robot to a decoy goal given a sensor alteration, demonstrating its polynomial-time complexity. We establish the computational hardness of optimizing sensor deception costs by providing a novel reduction from the Knapsack Problem. Furthermore, we formulate the optimal sensor deception problem as a Mixed Integer Linear Programming (MILP) model, offering a structured and scalable solution framework for generating deception strategies with optimal cost.

%%% Example
For example, consider a strategic defense scenario in a military base environment as shown in Fig.~\ref{fig:example}. An intruder ground robot, attempts to infiltrate an protected area containing ammunition, located in upper right cell, while avoiding detection. The environment contains 6 beacons, $S1$ to $S6$,  which the ground robot relies on for localization. The  defense system  of the base can alter the beacon identities by spoofing them, effectively misdirecting the robot away from the ammunition area and towards the middle cell containing a guard tower. The cost of beacon spoofing can include energy expenditure or the risk posed to authorized agents. This approach ensures that the deception remains undetected by the ground robot, reducing the risk of the intruder adapting its strategy in response to the environment’s defenses.


\textbf{Case Study:}


Figure~\ref{} presents a case-study example illustrating the sensor deception problem. In this scenario, two teams, $T_1$ and $T_2$, interact within a grid-based environment of size 7x7. Team $T_1$, spy team, consists of a single agent or robot, $r$, tasked with navigating from a designated start location, $Start$, to a goal location, $Goal$, while avoiding  guard agents from team $T_2$. Team $T_2$ comprises two guard agents, $a_1$ and $a_2$, that move randomly throughout the environment. The robot $r$ and the agents $a_1$, $a_2$ can move to any neighboring cell at each step, with their possible actions being $N, S, E,$ and $W$.  

The environment is equipped with three sensors, $S_1 (at [2,4]), S_2(at [4,2]),$ and $S_3(at [5,5])$, each having a perception range of two grid cells including the grid cell in which it resides. These sensors detect the presence of agents from $T_2$ and report an observation to $r$ whenever either $a_1$ or $a_2$ is within their range. Notably, sensors $S_1$ and $S_2$ have overlapping perception regions of 1-cell. To deceive the robot about their true locations, agents $a_1$ and $a_2$ can swap the identification of a pair of sensors.

\section{Related Work}
Deception of adversary or opponent by altering sensor information can be implemented in form of opacity \cite{opacity, JACOB2016135} and deceptive control \cite{zhang2022selection, milani-ssgattack-2020}, with our approach falling under the latter category. Deceptive control is implemented through adding, removal or altering sensors or observations. Placement of decoy targets is considered in \cite{fu-proactive-2023, milani-ssgattack-2020} with linear program solution to optimize deception. In \cite{fu-proactive-2023} utilizes probabilistic attack graphs unlike deterministic one in \cite{milani-ssgattack-2020}. Goal obfuscation considers hiding true goal among fake goals to implement deception \cite{goalobfuscation-2020, bernardini2020optimization}. A game theory based approach is used in deploying decoys for deception in \cite{kulkarni-decoy-2020, kulkarni-decoylabel-2020, li-games-2023}. In our method, we optimize  the alterations of sensors to lead the agent to  pre-determined decoy targets.

%and manipulating the cost of attack actions in probabilistic attack graphs and solves it as a bi-level linear program using a gradient ascent approach.

Markov Decision Process has been used in deceptive planning. Karabag et al. \cite{ufuk-2023} explore deception by an agent through partial observability of the supervisor, modeling the environment as an MDP. The agent optimizes the generation of a deceptive policy, quantifying deception using Kullback-Leibler (KL) divergence to ensure that the agent's actions remain indistinguishable from the supervisor's expectations while achieving its covert objective. In \cite{ufuk-2025}, the method is extended to team deception, where each agent is modeled as an MDP, and a centralized deceptive policy synthesis is applied while maintaining decentralized execution. In \cite{Savas_Verginis_Topcu_2022}, an agent deceives an adversary team about its true goal by modeling its behavior with MDPs and using Linear Programming to maximize deception, ensuring the highest probability of achieving its true goal. The observer’s predictions are formulated as probability distributions over true goals, guided by the maximum entropy principle. Ma et al. \cite{fu-covert-2024} investigate covert deception planning in a stochastic environment, modeled as an MDP, where the agent aims to maximize the discounted total reward while maintaining covert behavior. They employ a sequential likelihood ratio test and demonstrate that finite-memory policies can outperform Markovian policies in this constrained MDP framework. Due to the complexity of finite-memory policy search, the authors develop a primal-dual gradient-based method for synthesizing optimal and covert Markov policies.

Meira-Góes et al. \cite{Lafortune-2019} investigate sensor manipulation in a stochastic environment by modeling the system as a probabilistic automaton. The authors leverage concepts from stochastic games to synthesize an attack policy that maximizes the likelihood of the system being in an unsafe state. In \cite{Laforturne-2022}, the authors extend their work by modeling the interaction between the attacker and the system as an MDP, and also  incorporating penalties into the attack model as a second problem.

Anwar et. al. \cite{anwar-honeypot-2022} utilizes partially observable Markov decision process (POMDP) to model dynamical allocation of honeypots to trap attackers considering the partial observability in monitoring attackers.

%Although our method uses offline computation of sensor alteration before the execution of robot for efficiency with real time computations, it can be used in conjuction with online methods to account for dynamic changes and adaptability of the robot.
Our approach computes sensor alterations offline before any robot operations, and applicable to situations where online computations is not practical due to resource constraints. However, it can be used in conjunction with online approaches to increase robustness and adaptability in uncertain environments.

%Karabag et al. \cite{ufuk-2023} investigate deception by an agent by leveraging the supervisor's partial observability. The environment is modeled as an MDP, where the agent optimizes the generation of a deceptive policy. Deception is quantified using Kullback-Leibler (KL) divergence, ensuring that the agent's actions remain indistinguishable from the supervisor's expectations while achieving its covert objective. In \cite{ufuk-2025}, the method is extended to consider team deception where each is modeled as MDP, and considers centralized synthesis of deceptive policy while keeping the execution decentralized. In \cite{Savas_Verginis_Topcu_2022}, the agent deceives an adversary team about its true goal by modeling its behavior with MDPs and employing Linear Programming to maximize deception while ensuring the highest probability of achieving the true goal. The observer's predictions are generated as probability distributions over the true goals, guided by the maximum entropy principle. 
%Ma et. al. \cite{fu-covert-2024} considers covert deception planning in stochastic environment modeled as MDP that maximizes the discounted total reward  while maintaining covert behavior. They utilize a sequential-likelihood ratio test and prove that a finite-memory policy can be more effective than a Markovian policy in this constrained MDP framework. Given the complexity of the search space for finite-memory policies, the authors develop a primal-dual gradient-based search method for optimal and covert Markov policies.

Lv et. al. \cite{lv-ugv-2024} synthesize optimal deceptive strategy in a two-player game where one player have full observability and another partial.


